Seeing and hearing what has not been said; A multimodal client behavior classifier in Motivational Interviewing with interpretable fusion

Motivational Interviewing (MI) is an approach to therapy that emphasizes collaboration and encourages behavioral change. To evaluate the quality of an MI conversation, client utterances can be classified using the MISC code as either change talk, sustain talk, or follow/neutral talk. The proportion of change talk in a MI conversation is positively correlated with therapy outcomes, making accurate classification of client utterances essential. In this paper, we present a classifier that accurately distinguishes between the three MISC classes (change talk, sustain talk, and follow/neutral talk) leveraging multimodal features such as text, prosody, facial expressivity, and body expressivity. To train our model, we perform annotations on the publicly available AnnoMI dataset to collect multimodal information, including text, audio, facial expressivity, and body expressivity. Furthermore, we identify the most important modalities in the decision-making process, providing valuable insights into the interplay of different modalities during a MI conversation.

==> brouillon.tex <==
% \subsection{Plan : à enlever}
% \begin{itemize}
% \item MI coding correlated with therapy outcome \cite{magill2014technical,magill2018meta}
% \item automatic coding using only text explored \cite{howes2013using,ewbank2021understanding,chen2021feature,huang2018modeling}
% \item Facial expressions important \cite{pampouchidou2017automatic}
% \item multimodality begins to be explored
% \begin{itemize}
% \item prosodic features \cite{aswamenakul2018multimodal,singla2018using,tavabi2020multimodal}
% \item laughter  \cite{gupta2014predicting}
% \item facial expressions \cite{nakano2022detecting}
% \item explainability of important features \cite{singla2018using}
% \end{itemize}
% \item To our knowledge no body expressivity + no opensource
% \end{itemize}
% \subsection{Résumés citations : à enlever}
% \begin{itemize}
    
%     \item \cite{magill2014technical} : Therapist MI-consistent skills were correlated with more client language in favor of behavior change (i.e., change talk; r = .26, p < .0001), but not less client language against behavior change (i.e., sustain talk; r = .10, p = .09). MI-inconsistent skills were associated with less change talk (r = −.17, p = .001) as well as more sustain talk (r = .07, p = .009). Among these studies, client change talk was not associated with follow-up outcome (r = .06, p = .41), but sustain talk was associated with worse outcome (r = −.24, p = .001). In addition, studies that examined composite client language (e.g., an average of negative and positive statements) showed an overall positive relationship with client behavior change (r = .12, p = .006; k = 6).
% \item  \cite{magill2018meta} : , proportion MI consistency was
% related to higher proportion change talk (r = .11, p = .004) and higher proportion change talk
% was related to reductions in risk behavior at follow up (r = -.16, p < .001). When tested as two
% independent effects, client change talk was not significant, but sustain talk was positively
% associated with worse outcome (r = .19, p < .001)
% \end{itemize}
% Text only :
% \begin{itemize}
%     \item \cite{howes2013using} : Relationship with the therapeut correlated with therapy outcome. Use topic modelling (LDA) against manual coding of topics to predict therapy outcome : LDA good for therapeut client relationship while manual coding for therapy outcome
%     \item \cite{ewbank2021understanding} Use DL to classify CBT client utterances in 5 categories including change talk.
%     Our model reached human-level agreement on three of the five patient categories. Regression analyses revealed that increased counter change-talk (movement away from change) was associated with lower odds of both reliable improvement and engagement, while increased change-talk (movement towards change or self-exploration) was associated with increased odds of improvement and engagement.
%     \item \cite{chen2021feature} Predict CBT therapy outcome by combining word and utterance level featres. utterance level features are extracted from MI coding
%     \item \cite{huang2018modeling} Use bi-LSTM and topic modelling + timming within the session (begining or end)

% \end{itemize}
% Multimodal
% \begin{itemize}
%     \item \cite{aswamenakul2018multimodal} we perform statistical analyses on
% acoustic behavior descriptors to test their discriminatory powers.
% Then we utilize multimodality by combining acoustic features with
% linguistic features to improve the accuracy of client change talk
% prediction. Lastly, we investigate into our trained model to understand what features inform the model about client utterance class
% and gain insights into the nature of MISC codes, use LIWC
%     \item \cite{singla2018using} LSTM : prosody + text + attention weight : give the most important feature : at the word level
%     \item \cite{tavabi2020multimodal} : Use Bert and VGGish
%     \item \cite{pampouchidou2017automatic} Action Units can show some sign of depression
%     \item \cite{gupta2014predicting}We observe that our best model achieves
% an unweighted accuracy of 50.8% in a 3-way classification of
% positive vs negative valence ChangeTalk vs no ChangeTalk.
% Furthermore, we study the effect of including non-verbal behavior, specifically laughter, in our model. Information regarding
% location of laughter improves the unweighted accuracy of our
% model to 51.4\% and our experimental results suggest prosodic
% differences in laughter belonging to ChangeTalk utterances
% with different valences
%     \item \cite{nakano2022detecting} BiLSTM for Action units and text
% \end{itemize}
% \subsection{Vraie partie}

